From spin foams to area metric dynamics to gravitons

Although spin foams arose as quantizations of the length metric degrees of freedom, the quantum configuration space is rather based on areas as more fundamental variables. This is also highlighted by the semi-classical limit of four-dimensional spin foam models, which is described by the Area Regge action. Despite its central importance to spin foams the dynamics encoded by the Area Regge action is only poorly understood, in particular in the continuum limit. We perform here a systematic investigation of the dynamics defined by the Area Regge action on a regular centrally subdivided hypercubical lattice. This choice of lattice avoids many problems of the non-subdivided hypercubical lattice, for which the Area Regge action is singular. The regularity of the lattice allows to extract the continuum limit and its corrections, order by order in the lattice constant. We show that, contrary to widespread expectations which arose from the so-called flatness problem of spin foams, the continuum limit of the Area Regge action does describe to leading order the same graviton dynamics as general relativity. The next-to-leading order correction to the effective action for the length metric is of second order in the lattice constant, and is given by a quadratic term in the Weyl curvature tensor. This correction can be understood to originate from an underlying dynamics of area metrics. This suggests that the continuum limit of spin foam dynamics does lead to massless gravitons, and that the leading order quantum corrections can be understood to emerge from a generalization of the configuration space from length to area metrics.

==> Area Regge on regular lattice/Bibliography.tex <==
\begingroup
%\raggedright
\begin{thebibliography}{100}%\small

%\vspace{-2em}

\bibitem{BFCG2} S.~K.~Asante, B.~Dittrich, F.~Girelli, A.~Riello and P.~Tsimiklis,
  ``Quantum geometry from higher gauge theory,''
  arXiv:1908.05970 [gr-qc].
  %%CITATION = ARXIV:1908.05970;%%

\bibitem{EffSF1} S.~K.~Asante, B.~Dittrich and H.~M.~Haggard,
``Effective Spin Foam Models for Four-Dimensional Quantum Gravity,''
Phys. Rev. Lett. \textbf{125} (2020) no.23, 231301
%doi:10.1103/PhysRevLett.125.231301
[arXiv:2004.07013 [gr-qc]].

\bibitem{LQG} C. Rovelli,
\textit{Quantum Gravity},
(Cambridge University Press, Cambridge, 2004);
A. Ashtekar and J. Lewandowski,
``Background independent quantum gravity: a status report'',
Class. Quant. Grav. \textbf{21} R53 (2004), [arXiv:gr-qc/0404018];
T. ~Thiemann,
\textit{Introduction to Modern Canonical Quantum General Relativity},
(Cambridge University Press, Cambridge, 2007).
A.~Ashtekar and J.~Pullin,
\textit{Loop Quantum Gravity: The First 30 Years}, (World Scientific 2017)
%doi:10.1142/10445

\bibitem{Perez} A.~Perez,
  ``The Spin Foam Approach to Quantum Gravity,''
  Living Rev.\ Rel.\  {\bf 16} (2013) 3
 % doi:10.12942/lrr-2013-3
  [arXiv:1205.2019].
  %%CITATION = doi:10.12942/lrr-2013-3;%%

\bibitem{RyuTakayanagi} S.~Ryu and T.~Takayanagi, 
``Holographic Derivation of Entanglement Entropy from the anti--de Sitter Space/Conformal Field Theory Correspondence,''
Phys. Rev. Lett. {\bf 96} (2006) 181602.
%https://link.aps.org/doi/10.1103/PhysRevLett.96.181602

\bibitem{BHCounting} J.~D.~Bekenstein and V.~F.~Mukhanov,
  ``Spectroscopy of the quantum black hole,''
  Phys.\ Lett.\ B {\bf 360} (1995) 7
  %doi:10.1016/0370-2693(95)01148-J
  [gr-qc/9505012].
    A.~Ashtekar, J.~Baez, A.~Corichi and K.~Krasnov,
  ``Quantum geometry and black hole entropy,''
  Phys.\ Rev.\ Lett.\  {\bf 80} (1998) 904
 % doi:10.1103/PhysRevLett.80.904
  [gr-qc/9710007].
    J.~D.~Bekenstein,
  ``Statistics of black hole radiance and the horizon area spectrum,''
  Phys.\ Rev.\ D {\bf 91} (2015) no.12,  124052
 % doi:10.1103/PhysRevD.91.124052
  [arXiv:1505.03253 [gr-qc]].
  %%CITATION = doi:10.1103/PhysRevD.91.124052;%%
  J.~F.~Barbero G. and A.~Perez,
  ``Quantum Geometry and Black Holes,''
 % doi:10.1142/9789813220003_0008
  arXiv:1501.02963 [gr-qc].
  %%CITATION = doi:10.1142/9789813220003_0008;%%

\bibitem{Schuller1} F.~P.~Schuller and M.~N.~R.~Wohlfarth,
``Geometry of manifolds with area metric: multi-metric backgrounds,''
Nucl. Phys. B \textbf{747} (2006), 398-422
%doi:10.1016/j.nuclphysb.2006.04.019
[arXiv:hep-th/0508170 [hep-th]].

\bibitem{Schuller2} F.~P.~Schuller and M.~N.~R.~Wohlfarth,
``Canonical differential geometry of string backgrounds,''
JHEP \textbf{02} (2006), 059
%doi:10.1088/1126-6708/2006/02/059
[arXiv:hep-th/0511157 [hep-th]].
  R.~Punzi, F.~P.~Schuller and M.~N.~R.~Wohlfarth,
``Geometry for the accelerating universe,''
Phys. Rev. D \textbf{76} (2007), 101501
%doi:10.1103/PhysRevD.76.101501
[arXiv:hep-th/0612133 [hep-th]].
R.~Punzi, F.~P.~Schuller and M.~N.~R.~Wohlfarth,
``Area metric gravity and accelerating cosmology,''
JHEP \textbf{02} (2007), 030
%doi:10.1088/1126-6708/2007/02/030
[arXiv:hep-th/0612141 [hep-th]].

\bibitem{SFLimit} J.~W.~Barrett and R.~M.~Williams,
``The Asymptotics of an amplitude for the four simplex,''
Adv. Theor. Math. Phys. \textbf{3} (1999), 209-215
%doi:10.4310/ATMP.1999.v3.n2.a1
[arXiv:gr-qc/9809032 [gr-qc]].
F.~Conrady and L.~Freidel,
  ``On the semiclassical limit of 4d spin foam models,''
  Phys.\ Rev.\ D {\bf 78} (2008) 104023
  %doi:10.1103/PhysRevD.78.104023
  [arXiv:0809.2280 [gr-qc]].
  %%CITATION = doi:10.1103/PhysRevD.78.104023;%%
    J.~W.~Barrett, R.~J.~Dowdall, W.~J.~Fairbairn, H.~Gomes and F.~Hellmann,
  ``Asymptotic analysis of the EPRL four-simplex amplitude,''
  J.\ Math.\ Phys.\  {\bf 50} (2009) 112504
  doi:10.1063/1.3244218
  [arXiv:0902.1170 [gr-qc]];
  %%CITATION = doi:10.1063/1.3244218;%%
   J.~W.~Barrett, R.~J.~Dowdall, W.~J.~Fairbairn, F.~Hellmann and R.~Pereira,
  ``Lorentzian spin foam amplitudes: Graphical calculus and asymptotics,''
  Class.\ Quant.\ Grav.\  {\bf 27} (2010) 165009
  %doi:10.1088/0264-9381/27/16/165009
  [arXiv:0907.2440 [gr-qc]];
  %%CITATION = doi:10.1088/0264-9381/27/16/165009;%%
    M.~X.~Han and M.~Zhang,
  ``Asymptotics of Spinfoam Amplitude on Simplicial Manifold: Euclidean Theory,''
  Class.\ Quant.\ Grav.\  {\bf 29} (2012) 165004
 % doi:10.1088/0264-9381/29/16/165004
  [arXiv:1109.0500 [gr-qc]].
  %%CITATION = doi:10.1088/0264-9381/29/16/165004;%%


%

\bibitem{EffSF2} S.~K.~Asante, B.~Dittrich and H.~M.~Haggard,
``Discrete gravity dynamics from effective spin foams,''
Class. Quant. Grav. \textbf{38} (2021) no.14, 145023
%doi:10.1088/1361-6382/ac011b
[arXiv:2011.14468 [gr-qc]].

\bibitem{EffSF3} S.~K.~Asante, B.~Dittrich and J.~Padua-Arguelles,
``Effective spin foam models for Lorentzian quantum gravity,''
Class. Quant. Grav. \textbf{38} (2021) no.19, 195002
%doi:10.1088/1361-6382/ac1b44
[arXiv:2104.00485 [gr-qc]].

\bibitem{AreaRegge} C.~Rovelli,
``The Basis of the Ponzano-Regge-Turaev-Viro-Ooguri quantum gravity model in the loop representation basis,''
Phys. Rev. D \textbf{48} (1993), 2702-2707
%doi:10.1103/PhysRevD.48.2702
[arXiv:hep-th/9304164 [hep-th]].
J.~W.~Barrett, M.~Rocek and R.~M.~Williams,
  ``A Note on area variables in Regge calculus,''
  Class.\ Quant.\ Grav.\  {\bf 16} (1999) 1373
  %doi:10.1088/0264-9381/16/4/025
  [gr-qc/9710056];
  %%CITATION = doi:10.1088/0264-9381/16/4/025;%%

\bibitem{Regge} T.~Regge,
  ``General Relativity Without Coordinates,''
Nuovo Cim.  {\bf 19} (1961) 558.
  %doi:10.1007/BF02733251
  %%CITATION = doi:10.1007/BF02733251;%%

\bibitem{flatness} V.~Bonzom,
  ``Spin foam models for quantum gravity from lattice path integrals,''
  Phys.\ Rev.\ D {\bf 80} (2009) 064028
  %doi:10.1103/PhysRevD.80.064028
  [arXiv:0905.1501 [gr-qc]].
  %%CITATION = doi:10.1103/PhysRevD.80.064028;%%
   F.~Hellmann and W.~Kaminski,
  ``Holonomy spin foam models: Asymptotic geometry of the partition function,''
  JHEP {\bf 1310} (2013) 165
 % doi:10.1007/JHEP10(2013)165
  [arXiv:1307.1679 [gr-qc]].
  %%CITATION = doi:10.1007/JHEP10(2013)165;%%
    J.~R.~Oliveira,
  ``EPRL/FK Asymptotics and the Flatness Problem,''
  Class.\ Quant.\ Grav.\  {\bf 35} (2018) no.9,  095003
%  doi:10.1088/1361-6382/aaae82
  [arXiv:1704.04817 [gr-qc]].
   P.~Don\`a, F.~Gozzini and G.~Sarno,
  ``Searching for classical geometries in spin foam amplitudes: a numerical method,''
 % doi:10.1088/1361-6382/ab7ee1
  arXiv:1909.07832 [gr-qc].
  %%CITATION = doi:10.1088/1361-6382/ab7ee1;%%
J.~Engle, W.~Kaminski and J.~Oliveira,
``Addendum: EPRL/FK Asymptotics and the Flatness Problem,''
[arXiv:2012.14822 [gr-qc]].

\bibitem{MuxinSmallBI} M.~Han,
``On Spinfoam Models in Large Spin Regime,''
Class. Quant. Grav. \textbf{31} (2014), 015004
%doi:10.1088/0264-9381/31/1/015004
[arXiv:1304.5627 [gr-qc]].
M.~Han,
``Semiclassical Analysis of Spinfoam Model with a Small Barbero-Immirzi Parameter,''
Phys. Rev. D \textbf{88} (2013), 044051
doi:10.1103/PhysRevD.88.044051
[arXiv:1304.5628 [gr-qc]].

\bibitem{ComplexSP} M.~Han, Z.~Huang, H.~Liu and D.~Qu,
``Complex critical points and curved geometries in four-dimensional Lorentzian spinfoam quantum gravity,''
[arXiv:2110.10670 [gr-qc]].

\bibitem{DittrichRyan} B.~Dittrich and J.~P.~Ryan,
  ``Phase space descriptions for simplicial 4d geometries,''
  Class.\ Quant.\ Grav.\  {\bf 28} (2011) 065006
 % doi:10.1088/0264-9381/28/6/065006
  [arXiv:0807.2806 [gr-qc]];
  B.~Dittrich and J.~P.~Ryan,
  ``Simplicity in simplicial phase space,''
  Phys.\ Rev.\ D {\bf 82} (2010) 064026
 % doi:10.1103/PhysRevD.82.064026
  [arXiv:1006.4295 [gr-qc]].
  %%CITATION = doi:10.1103/PhysRevD.82.064026;%%
  ``On the role of the Barbero-Immirzi parameter in discrete quantum gravity,''
  Class.\ Quant.\ Grav.\  {\bf 30} (2013) 095015
%  doi:10.1088/0264-9381/30/9/095015
  [arXiv:1209.4892 [gr-qc]].

\bibitem{BC} J.~W.~Barrett and L.~Crane,
``Relativistic spin networks and quantum gravity,''
J. Math. Phys. \textbf{39} (1998), 3296-3302
%doi:10.1063/1.532254
[arXiv:gr-qc/9709028 [gr-qc]].

\bibitem{EPRL-FK} J.~Engle, R.~Pereira and C.~Rovelli,
  ``The Loop-quantum-gravity vertex-amplitude,''
  Phys.\ Rev.\ Lett.\  {\bf 99} (2007) 161301
 % doi:10.1103/PhysRevLett.99.161301
  [arXiv:0705.2388 [gr-qc]];
  %%CITATION = doi:10.1103/PhysRevLett.99.161301;%%
  L.~Freidel and K.~Krasnov,
  ``A New Spin Foam Model for 4d Gravity,''
  Class.\ Quant.\ Grav.\  {\bf 25} (2008) 125018
  %doi:10.1088/0264-9381/25/12/125018
  [arXiv:0708.1595 [gr-qc]];
       E.~R.~Livine and S.~Speziale,
  ``Consistently Solving the Simplicity Constraints for Spinfoam Quantum Gravity,''
  EPL {\bf 81} (2008) no.5,  50004
 % doi:10.1209/0295-5075/81/50004
  [arXiv:0708.1915 [gr-qc]];
  %%CITATION = doi:10.1088/0264-9381/25/12/125018;%%
    J.~Engle, E.~Livine, R.~Pereira and C.~Rovelli,
  ``LQG vertex with finite Immirzi parameter,''
  Nucl.\ Phys.\ B {\bf 799} (2008) 136
  %doi:10.1016/j.nuclphysb.2008.02.018
  [arXiv:0711.0146 [gr-qc]];
  %%CITATION = doi:10.1016/j.nuclphysb.2008.02.018;%%
  A.~Baratin and D.~Oriti,
``Group field theory and simplicial gravity path integrals: A model for Holst-Plebanski gravity,''
Phys. Rev. D \textbf{85} (2012), 044003
%doi:10.1103/PhysRevD.85.044003
[arXiv:1111.5842 [hep-th]].

\bibitem{ARE1} B.~Dittrich,
``Modified Graviton Dynamics From Spin Foams: The Area Regge Action,''
[arXiv:2105.10808 [gr-qc]].

\bibitem{ReggeWilliams} T.~Regge and R.~M.~Williams,
``Discrete structures in gravity,''
J. Math. Phys. \textbf{41} (2000), 3964-3984
%doi:10.1063/1.533333
[arXiv:gr-qc/0012035 [gr-qc]].

\bibitem{LinkNB} {\href{https://github.com/star-pirate/Centrally_Subdivided_Area_Regge}{ Link to GitHub Repository}}

\bibitem{RocekWilliams} M.~Rocek and R.~M.~Williams,
``Quantum Regge Calculus,''
Phys. Lett. B \textbf{104} (1981), 31.
%doi:10.1016/0370-2693(81)90848-0
M.~Rocek and R.~M.~Williams,
``The Quantization of Regge Calculus,''
Z. Phys. C \textbf{21} (1984), 371 .
%doi:10.1007/BF01581603

\bibitem{Hol3D4D} V.~Bonzom and B.~Dittrich,
``3D holography: from discretum to continuum,''
JHEP \textbf{03} (2016), 208
%doi:10.1007/JHEP03(2016)208
[arXiv:1511.05441 [hep-th]].
S.~K.~Asante, B.~Dittrich and H.~M.~Haggard,
``Holographic description of boundary gravitons in (3+1) dimensions,''
JHEP \textbf{01} (2019), 144
%doi:10.1007/JHEP01(2019)144
[arXiv:1811.11744 [hep-th]].

\bibitem{PImeasure1} B.~Dittrich and S.~Steinhaus,
  ``Path integral measure and triangulation independence in discrete gravity,''
  Phys.\ Rev.\ D {\bf 85} (2012) 044032
 % doi:10.1103/PhysRevD.85.044032
  [arXiv:1110.6866 [gr-qc]];
  %%CITATION = doi:10.1103/PhysRevD.85.044032;%%
  B.~Dittrich, W.~Kami\'nski and S.~Steinhaus,
``Discretization independence implies non-locality in 4D discrete quantum gravity,''
Class. Quant. Grav. \textbf{31} (2014) no.24, 245009
%doi:10.1088/0264-9381/31/24/245009
[arXiv:1404.5288 [gr-qc]].
S.~K.~Asante and B.~Dittrich,
``Perfect discretizations as a gateway to one-loop partition functions for 4D gravity,''
[arXiv:2112.03307 [gr-qc]].

\bibitem{Improved} B.~Bahr and B.~Dittrich,
``Improved and Perfect Actions in Discrete Gravity,''
Phys. Rev. D \textbf{80} (2009), 124030
%doi:10.1103/PhysRevD.80.124030
[arXiv:0907.4323 [gr-qc]].

\bibitem{BahrDittrichHe} B.~Bahr, B.~Dittrich and S.~He,
``Coarse graining free theories with gauge symmetries: the linearized case,''
New J. Phys. \textbf{13} (2011), 045009
%doi:10.1088/1367-2630/13/4/045009
[arXiv:1011.3667 [gr-qc]].





%

\bibitem{ContLimit} B.~Dittrich,
``The continuum limit of loop quantum gravity - a framework for solving the theory,''
doi:10.1142/9789813220003\_0006
[arXiv:1409.1450 [gr-qc]].
B.~Dittrich, F.~C.~Eckert and M.~Martin-Benito,
``Coarse graining methods for spin net and spin foam models,''
New J. Phys. \textbf{14} (2012), 035008
%doi:10.1088/1367-2630/14/3/035008
[arXiv:1109.4927 [gr-qc]].
C.~Delcamp and B.~Dittrich,
``Towards a phase diagram for spin foams,''
Class. Quant. Grav. \textbf{34} (2017) no.22, 225006
%doi:10.1088/1361-6382/aa8f24
[arXiv:1612.04506 [gr-qc]].
 S.~Steinhaus,
``Coarse Graining Spin Foam Quantum Gravity\textemdash{}A Review,''
Front. in Phys. \textbf{8} (2020), 295
%doi:10.3389/fphy.2020.00295
[arXiv:2007.01315 [gr-qc]].

\bibitem{ADH1} S.~K.~Asante, B.~Dittrich and H.~M.~Haggard,
  ``The Degrees of Freedom of Area Regge Calculus: Dynamics, Non-metricity, and Broken Diffeomorphisms,''
  Class.\ Quant.\ Grav.\  {\bf 35} (2018) no.13,  135009
 % doi:10.1088/1361-6382/aac588
  [arXiv:1802.09551]
  %%CITATION = doi:10.1088/1361-6382/aac588;%%

\bibitem{AreaAngle} B.~Dittrich and S.~Speziale,
  ``Area-angle variables for general relativity,''
  New J.\ Phys.\  {\bf 10} (2008) 083006
%  doi:10.1088/1367-2630/10/8/083006
  [arXiv:0802.0864 [gr-qc]].
  %%CITATION = doi:10.1088/1367-2630/10/8/083006;%%

\bibitem{DittrichHoehn1} B.~Dittrich and P.~A.~H\"ohn,
  ``Canonical simplicial gravity,''
  Class. Quant. Grav.  {\bf 29} (2012) 115009
 % doi:10.1088/0264-9381/29/11/115009
  [arXiv:1108.1974 [gr-qc]].
  %%CITATION = doi:10.1088/0264-9381/29/11/115009;%%
B.~Dittrich and P.~A.~H\"ohn,
``Constraint analysis for variational discrete systems,''
J. Math. Phys. \textbf{54} (2013), 093505
%doi:10.1063/1.4818895
[arXiv:1303.4294 [math-ph]].

\bibitem{Mara} P.~S.~Mara, ``Triangulations for the cube" Journal of Combinatorical Theory (A) {\bf 20} (1976) 170

\bibitem{DittrichFreidelSpeziale} B.~Dittrich, L.~Freidel and S.~Speziale,
``Linearized dynamics from the 4-simplex Regge action,''
Phys. Rev. D \textbf{76} (2007), 104020
%doi:10.1103/PhysRevD.76.104020
[arXiv:0707.4513 [gr-qc]].

\bibitem{DiffReview08} B.~Dittrich,
``Diffeomorphism symmetry in quantum gravity models,''
Adv. Sci. Lett. \textbf{2}, 151
%doi:10.1166/asl.2009.1022
[arXiv:0810.3594 [gr-qc]].

\bibitem{BarrettWilliams} J.~W.~Barrett,
``The fundamental theorem of linearized Regge calculus,''
Phys. Lett. B \textbf{190} (1987), 135-136.
%doi:10.1016/0370-2693(87)90853-7
J.~W.~Barrett and R.~M.~Williams,
``The Convergence of Lattice Solutions of Linearized Regge Calculus,''
Class. Quant. Grav. \textbf{5} (1988), 1543-1556.
%doi:10.1088/0264-9381/5/12/007

\bibitem{Wainwright} C.~Wainwright and R.~M.~Williams,
``Area Regge calculus and discontinuous metrics,''
Class. Quant. Grav. \textbf{21} (2004), 4865-4880
%doi:10.1088/0264-9381/21/21/008
[arXiv:gr-qc/0405031 [gr-qc]].

\bibitem{HamberWilliamsHO} H.~W.~Hamber and R.~M.~Williams,
``Simplicial Quantum Gravity With Higher Derivative Terms: Formalism and Numerical Results in Four-dimensions,''
Nucl. Phys. B \textbf{269} (1986), 712-743
%doi:10.1016/0550-3213(86)90518-3

\bibitem{PerfectPI} B.~Bahr, B.~Dittrich and S.~Steinhaus,
``Perfect discretization of reparametrization invariant path integrals,''
Phys. Rev. D \textbf{83} (2011), 105026
doi:10.1103/PhysRevD.83.105026
[arXiv:1101.4775 [gr-qc]].

\bibitem{Krasnov} K.~Krasnov,
  ``Gravity as BF theory plus potential,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 24} (2009) 2776
  %doi:10.1142/S0217751X09046151
  [arXiv:0907.4064 [gr-qc]];
  %%CITATION = doi:10.1142/S0217751X09046151;%%
    K.~Krasnov,
  ``Effective metric Lagrangians from an underlying theory with two propagating degrees of freedom,''
  Phys.\ Rev.\ D {\bf 81} (2010) 084026
 % doi:10.1103/PhysRevD.81.084026
  [arXiv:0911.4903 [hep-th]].
  %%CITATION = doi:10.1103/PhysRevD.81.084026;%%

\bibitem{Alesci} E.~Alesci and C.~Rovelli,
``The Complete LQG propagator. I. Difficulties with the Barrett-Crane vertex,''
Phys. Rev. D \textbf{76} (2007), 104012
%doi:10.1103/PhysRevD.76.104012
[arXiv:0708.0883 [gr-qc]].

\bibitem{DG} B.~Dittrich and M.~Geiller,
``A new vacuum for Loop Quantum Gravity,''
Class. Quant. Grav. \textbf{32} (2015) no.11, 112001
%doi:10.1088/0264-9381/32/11/112001
[arXiv:1401.6441 [gr-qc]].
B.~Bahr, B.~Dittrich and M.~Geiller,
``A new realization of quantum geometry,''
Class. Quant. Grav. \textbf{38} (2021) no.14, 145021
%doi:10.1088/1361-6382/abfed1
[arXiv:1506.08571 [gr-qc]].

\bibitem{SFDiv} C.~Perini, C.~Rovelli and S.~Speziale,
``Self-energy and vertex radiative corrections in LQG,''
Phys. Lett. B \textbf{682} (2009), 78-84
%doi:10.1016/j.physletb.2009.10.076
[arXiv:0810.1714 [gr-qc]].
A.~Riello,
``Self-energy of the Lorentzian Engle-Pereira-Rovelli-Livine and Freidel-Krasnov model of quantum gravity,''
Phys. Rev. D \textbf{88} (2013) no.2, 024011
%doi:10.1103/PhysRevD.88.024011
[arXiv:1302.1781 [gr-qc]].
V.~Bonzom and B.~Dittrich,
``Bubble divergences and gauge symmetries in spin foams,''
Phys. Rev. D \textbf{88} (2013), 124021
%doi:10.1103/PhysRevD.88.124021
[arXiv:1304.6632 [gr-qc]].
L.~Q.~Chen,
``Bulk amplitude and degree of divergence in 4d spin foams,''
Phys. Rev. D \textbf{94} (2016) no.10, 104025
%doi:10.1103/PhysRevD.94.104025
[arXiv:1602.01825 [gr-qc]].

\bibitem{DiffDiv} B.~Bahr and B.~Dittrich,
``(Broken) Gauge Symmetries and Constraints in Regge Calculus,''
Class. Quant. Grav. \textbf{26} (2009), 225011
%doi:10.1088/0264-9381/26/22/225011
[arXiv:0905.1670 [gr-qc]].
B.~Bahr and B.~Dittrich,
``Breaking and restoring of diffeomorphism symmetry in discrete gravity,''
AIP Conf. Proc. \textbf{1196} (2009) no.1, 10
%doi:10.1063/1.3284371
[arXiv:0909.5688 [gr-qc]].

\bibitem{BahrStein} B.~Bahr and S.~Steinhaus,
``Numerical evidence for a phase transition in 4d spin foam quantum gravity,''
Phys. Rev. Lett. \textbf{117} (2016) no.14, 141302
%doi:10.1103/PhysRevLett.117.141302
[arXiv:1605.07649 [gr-qc]].

\bibitem{Ambjorn:1997ub} J.~Ambjorn, J.~L.~Nielsen, J.~Rolf and G.~K.~Savvidy,
%``Spikes in quantum Regge calculus,''
Class. Quant. Grav. \textbf{14} (1997), 3225-3241
doi:10.1088/0264-9381/14/12/009
[arXiv:gr-qc/9704079 [gr-qc]].

\bibitem{Gibbons:1978ac} G.~W.~Gibbons, S.~W.~Hawking and M.~J.~Perry,
``Path Integrals and the Indefiniteness of the Gravitational Action,''
Nucl. Phys. B \textbf{138} (1978), 141-150

\bibitem{LollLR} R.~Loll,
``Discrete approaches to quantum gravity in four-dimensions,''
Living Rev. Rel. \textbf{1} (1998), 13
%doi:10.12942/lrr-1998-13

\bibitem{LorCal} J.~Feldbrugge, J.~L.~Lehners and N.~Turok,
``Lorentzian Quantum Cosmology,''
Phys. Rev. D \textbf{95} (2017) no.10, 103508
%doi:10.1103/PhysRevD.95.103508
[arXiv:1703.02076 [hep-th]].
M.~Han, Z.~Huang, H.~Liu, D.~Qu and Y.~Wan,
``Spinfoam on a Lefschetz thimble: Markov chain Monte Carlo computation of a Lorentzian spinfoam propagator,''
Phys. Rev. D \textbf{103} (2021) no.8, 084026
%doi:10.1103/PhysRevD.103.084026
[arXiv:2012.11515 [gr-qc]].
D.~Jia,
``Complex, Lorentzian, and Euclidean simplicial quantum gravity: numerical methods and physical prospects,''
[arXiv:2110.05953 [gr-qc]].
S.~K.~Asante, B.~Dittrich and J.~Padua-Arg\"uelles,
``Complex actions and causality violations: Applications to Lorentzian quantum cosmology,''
[arXiv:2112.15387 [gr-qc]].


\end{thebibliography}\endgroup

